Pruning One More Token is Enough: Leveraging Latency-Workload Non-Linearities for Vision Transformers on the Edge

This paper investigates how to efficiently deploy vision transformers on edge devices for small workloads. Recent methods reduce the latency of transformer neural networks by removing or merging tokens, with small accuracy degradation. However, these methods are not designed with edge device deployment in mind: they do not leverage information about the latency-workload trends to improve efficiency. We address this shortcoming in our work. First, we identify factors that affect ViT latency-workload relationships. Second, we determine token pruning schedule by leveraging non-linear latency-workload relationships. Third, we demonstrate a training-free, token pruning method utilizing this schedule. We show other methods may increase latency by 2-30%, while we reduce latency by 9-26%. For similar latency (within 5.2% or 7ms) across devices we achieve 78.6%-84.5% ImageNet1K accuracy, while the state-of-the-art, Token Merging, achieves 45.8%-85.4%.

==> tables/table_anomaly_latency.tex <==
%%% PURPOSE ? 
%%% Have a table that shows when token pruning can actually DEGRADE latency!
%%% Includes our method, but also shows some instances where 
\begin{table}[!t]
    \centering
    \setlength{\tabcolsep}{8pt}
    \setlength{\belowcaptionskip}{-8pt}
    %%% Device, Model + Wrapper, Accuracy, Latency
    \begin{tabular}{llrr}
        \toprule
        \textbf{Device} & \textbf{Method} & $\downarrow$\textbf{Top-1} & $\downarrow$\textbf{Median}\\
        ~ & & \textbf{Loss} & \textbf{Latency (ms)}\\
        \toprule
        %%%% TX2
        \multirow{4}{*}{TX2} & Baseline & ~ & \phantom{(-0.00\%)} 35.32\\ 
         & Top-K \hfill(r=6) & 0.73 & \textcolor{red}{(+18.6\%)} 43.38\\
         & ToMe \hfill(r=6) & 0.27 & \textcolor{red}{(+30.3\%)} 50.70\\
         & Ours \hfill(R=69) & 0.99 & \textcolor{blue}{(-9.06\%)} 32.12\\
        \bottomrule
    \end{tabular}
    \caption{
    Experiment that illustrates pruning overhead.
    Given comparable total pruned tokens (69 to 72), for certain workload sizes a token pruning mechanism may \textit{increase} latency due to the overhead of performing pruning at multiple layers.
    Our pruning method is applied at a single layer to avoid this overhead.
    }
    \label{tab:latency_anomaly}
\end{table}

==> tables/table_baseline_data.tex <==
\begin{table}[h!]
\begin{tabular}{ccrc}
Model                        & Batch Size & Latency(ms) & Accuracy \\ \hline
%%% Deit-B-dist
%\multirow{4}{*}{DeiT-B-dist} & 1          & 82        & \multirow{4}{*}{83.25}\\
%                             & 2          & 164       &             \\
%                             & 4          & 302       &             \\
%                             & 8          & 570       &             \\ \hline
%%% DeiT-S-dist
%\multirow{4}{*}{DeiT-S-dist} & 1          & 30       & \multirow{4}{*}{ 81.04}\\
%                             & 2          & 55       &              \\
%                             & 4          & 99       &              \\
%                             & 8          & 184      &              \\ \hline
%%% DeiT-S
\multirow{4}{*}{DeiT-S}      & 1          & 30       & \multirow{4}{*}{79.76}\\
                             & 2          & 55       &              \\
                             & 4          & 99       &              \\
                             & 8          & 185      &             \\ \hline
%%% DeiT-B
\multirow{4}{*}{DeiT-B}      & 1          & 82       & \multirow{4}{*}{ 81.74}\\
                             & 2          & 164      &             \\
                             & 4          & 298      &             \\
                             & 8          & 559      &             \\ \hline
\end{tabular}
\caption{Baseline accuracy and latency measurements for the DeiT \cite{touvron_training_2021} architectures we use. Pre-trained models are obtained from TIMM \cite{huggingface_timm}. Latency was measured on a NVIDIA Jetson TX2, a commodity edge device.}
\label{tab:baseline_data}
\end{table}

==> tables/table_cvpr2024_eval_all_results.tex <==
%%%
%%% Accuracy table
%%%
\setlength{\arrayrulewidth}{0.30mm}
\begin{table*}[t]
\centering
%\setlength{\extrarowheight}{0.5pt}
    \begin{tabular}{clrrrr}
        %%% Header
        \toprule
        & & \multicolumn{4}{c}{IM1K Accuracy (\%) for Batch Size}\\
        \multicolumn{1}{l}{Model} & Method & 1 & 2 & 4 & 8 \\
        \toprule
        %%%
        %%% DeiT-S
        %%%
        \multicolumn{1}{c}{\multirow{6}{*}{DeiT-S}} & \cellcolor{gray!20!white}\textbf{Baseline} & \cellcolor{gray!20!white}79.76 & \cellcolor{gray!20!white}79.76 & \cellcolor{gray!20!white}79.76 & \cellcolor{gray!20!white}79.76 \\
        %%% Ours
        \multicolumn{1}{c}{} & Ours & 78.75 (-1.01) & 78.54 (-1.22) & 77.32 (-2.44) & 77.32 (-2.44)\\
        %%% DynamicViT
        \multicolumn{1}{c}{} & DynamicViT(r=0.7) & 79.30 (-0.46) & 79.30 (-0.46) & 79.30 (-0.46) & 79.30 (-0.46)\\
        %%% Modified DynamicViT
        %\multicolumn{1}{c}{} & DynamicViT* & 78.96 (-0.80) & 78.49 (-1.27) & 75.76 (-4.00) &  75.76 (-4.00)\\
        \multicolumn{1}{c}{} & DynamicViT* & 79.04 (-0.72) & 78.83 (-0.93) & 77.65 (-2.11) &  77.65 (-2.11)\\
        %%% ToMe(r=18)
        \multicolumn{1}{c}{} & ToMe(r=18) & 76.42 (-3.34) & 76.42 (-3.34) & 76.42 (-3.34) & 76.42 (-3.34)\\
        %%% ToMe modified)
        \multicolumn{1}{c}{} & ToMe* & 78.49 (-1.27) & 78.13 (-1.63) & 74.05 (-5.71) & 74.05 (-5.71)\\
        \midrule
        %%%
        %%% DeiT-B
        %%%
        \multicolumn{1}{c}{\multirow{6}{*}{DeiT-B}} & \cellcolor{gray!20!white}\textbf{Baseline} & \cellcolor{gray!20!white}81.74 & \cellcolor{gray!20!white}81.74 & \cellcolor{gray!20!white}81.74 & \cellcolor{gray!20!white}81.74 \\
        %%% Ours
        \multicolumn{1}{c}{} & Ours & 80.58 (-1.16) & 80.58 (-1.16) & 78.98 (-2.76) & 77.28 (-4.46) \\
        %%% DynamicViT
        \multicolumn{1}{c}{} & DynamicViT(r=0.7) & 81.44 (-0.30) & 81.44 (-0.30) & 81.44 (-0.30) & 81.44 (-0.30)\\
        %\multicolumn{1}{c}{} & DynamicViT* & 80.81 (-0.93) & 80.81 (-0.93) & 76.69 (-5.05) & 69.94 (-11.8) \\
        \multicolumn{1}{c}{} & DynamicViT* & 81.22 (-0.52) & 81.22 (-0.52) & 79.90 (-1.84) & 78.67 (-3.07) \\
        \multicolumn{1}{c}{} & ToMe(r=13) & 79.69 (-2.05) & 79.69 (-2.05) & 79.69 (-2.05) & 79.69 (-2.05)\\
        \multicolumn{1}{c}{} & ToMe* & 79.59 (-2.15) & 79.59 (-2.15) & 75.42 (-6.32) & 74.49 (-7.25)\\
        \bottomrule
    \end{tabular}
    %%% Caption
    \caption{\NJE{HIGH PRIO: Remove, emulate Fig. 4 style and duplicate for all three devices}
    Accuracy evaluation and comparison of our method, existing techniques, and existing techniques augmented with our schedule (*).
    %\JD{I usually see table captions above the table (move caption to above the table declaration). Maybe that is not the custom at CVPR though. Check a prior paper.}
    }
    \label{tab:eval_accuracy}
\end{table*}

%%%
%%% Latency Table
%%%
\setlength{\arrayrulewidth}{0.30mm}
\begin{table*}
\centering
%\setlength{\extrarowheight}{0.5pt}
    \begin{tabular}{clrrrr}
        %%% Header
        \toprule
        & & \multicolumn{4}{c}{Latency (ms) for Batch Size}\\
        \multicolumn{1}{l}{Model} & Method & 1 & 2 & 4 & 8 \\
        \toprule
        %%%
        %%% DeiT-S
        %%%
        \multicolumn{1}{c}{\multirow{6}{*}{DeiT-S}} & \cellcolor{gray!20!white}\textbf{Baseline} & \cellcolor{gray!20!white}30.40 & \cellcolor{gray!20!white}55.36 & \cellcolor{gray!20!white}99.12 & \cellcolor{gray!20!white}184.6\\
        \multicolumn{1}{c}{} & Ours & \textbf{28.67 (-5.70\%)} & \textbf{41.5 (-25.0\%)} & 65.0 (-34.4\%) & 117.4 (-36.4\%)\\
        \multicolumn{1}{c}{} & DynamicViT(r=0.7) & 38.71 (+27.3\%) & 55.24 (-0.22\%) & 92.83 (-6.35\%) & 168.7 (-8.61\%)\\
        %\multicolumn{1}{c}{} & DynamicViT* & 38.66 (+27.2\%) & 47.04 (-15.0\%) & 69.07 (-30.3\%) & 121.7 (-34.1\%) \\
        \multicolumn{1}{c}{} & DynamicViT* & 33.04 (+8.68\%) & 52.95 (-4.35\%) & 86.89 (-12.3\%) & 159.2 (-13.8\%) \\
        \multicolumn{1}{c}{} & ToMe(r=18) & 44.43 (+46.2\%) & 50.35 (+9.05\%) & 58.3 (-41.2\%) & \textbf{95.92 (-48.0\%)}\\
        \multicolumn{1}{c}{} & ToMe* & 31.56 (+3.82\%) & 42.31 (-23.6\%) & \textbf{56.93 (-42.6\%)} & 106.7 (-42.2\%)\\
        \midrule
        %%%
        %%% DeiT-B
        %%%
        \multicolumn{1}{c}{\multirow{6}{*}{DeiT-B}} & \cellcolor{gray!20!white}\textbf{Baseline} & \cellcolor{gray!20!white}82.09 & \cellcolor{gray!20!white}163.7 & \cellcolor{gray!20!white}297.6 & \cellcolor{gray!20!white}558.7\\
        \multicolumn{1}{c}{} & Ours & \textbf{59.65 (-27.3\%)} & 111.6 (-31.2\%) & 187.3 (-37.1\%) & 319.33 (-42.8\%)\\
        \multicolumn{1}{c}{} & DynamicViT(r=0.7) & 89.07 (+8.50\%) & 159.9 (-2.32\%) & 276.5 (-7.09\%) & 512.9 (-8.20\%)\\
        %\multicolumn{1}{c}{} & DynamicViT* & 74.95 (-8.70\%) & 134.1 (-18.1\%) & 121.7 (-59.1\%) & 229.5 (-58.9\%) \\
        \multicolumn{1}{c}{} & DynamicViT* & 80.52 (-1.91\%) & 152.5 (-6.84\%) & 259.7 (-12.7\%) & 457.66 (-18.1\%) \\
        \multicolumn{1}{c}{} & ToMe(r=13) & 63.23 (-23.0\%) & 105.4 (-35.6\%) & 186.5 (-37.3\%) & 349.4 (-37.5\%) \\
        \multicolumn{1}{c}{} & ToMe* & 60.71 (-26.0\%) & \textbf{103.5 (-36.8\%)} & \textbf{165.0 (-44.6\%)} & \textbf{284.4 (-49.1\%)} \\
        \bottomrule
    \end{tabular}
    %%% Caption
    \caption{\NJE{TODO:  Remove and turn it into a scatter plot as in Fig. 5} Latency evaluation and comparison of our method, existing techniques, and existing techniques augmented with our schedule (*).}
    \label{tab:eval_latency}
\end{table*}
%%%
%%% Old Caption + Comments
%%%
%\caption{\JD{Add \% diff wrt. baseline} \NJE{Update DeiT-B ToMe r=18 to use r=16 - its a fairer benchmark}\PJ{Gaowen: Can you make two tables?}Evaluation and comparison of our method with ToMe and DynamicViT on a NVIDIA Jetson TX2. Baseline results are shown in Table \ref{tab:deit_baseline}. Colored cells indicate the smallest latency for a given batch size. \PJ{Jamie: Can you use a plot instead?} \PJ{YHL: Can you put latency all together, and accuracy together? Make some of the names smaller Use math font? replace "batch size" by "size". Careful about precision some have double and some have single You do not need to spell {Diet-S-dist} everywhere.}}

==> tables/table_large_workload.tex <==
\begin{table}[!ht]
    \centering
    \setlength{\tabcolsep}{4pt}
    \setlength{\belowcaptionskip}{0pt}
    %%% Device, Model + Wrapper, Accuracy, Latency
    \begin{tabular}{lllrrr}
        \toprule
        \textbf{Device} & \textbf{Batch} & \textbf{Model \&} & \textbf{Acc.} & \textbf{Median} \\
        ~ & \textbf{Size} & \textbf{Method} & \textbf{Loss} & \textbf{Latency (ms)}\\
        \toprule
        %%%
        %%% A100
        %%%
        %%% Batch Size 16
         \multirow{4}{*}{A100} & \multirow{4}{*}{16} & Top-K r=8 & 14.3 & \textcolor{blue}{(-52\%)} 74.4\\
         & & ToMe r=8 & 45.9 & \textcolor{blue}{(-52\%)} 73.9\\
         & & Ours R=185 & 15.7 & \textcolor{blue}{(-54\%)} 71.4\\
         & & \textbf{DinoV2-G} & ~ & \phantom{(-00\%)} 155.0\\
         \midrule
    \end{tabular}
    \caption{
    Evaluation of a DinoV2-G on an A100 system with a relatively large workload size (batch size 16). Hyperparameters of Top-K and ToMe were chosen to match the latency of our method.
    }
    \label{tab:large_workload}
\end{table}

==> tables/table_max_staircase_latency_reduce.tex <==
%%%
%%% Staircase Data %
%%% 
%%%
%%% Table: Hardware Aware Pruning Schedule Compared with ToMe (r=12, r=8)
%%%
%\setlength{\arrayrulewidth}{0.30mm}
%\begin{table}
 %   \centering
 %   \begin{tabular}{ccc}
 %   Model & Batch Size & Max Latency Reduction (\%)\\ \hline
    %%% Deit-B-dist
 %   \multirow{5}{*}{DeiT-S}         & 1 & 16.1\\
 %                                   & 2 & 19.7\\
 %                                   & 4 & 14.6\\
 %                                   & 8 & 10.5\\ \hline
    %                                & 16 & 8.11\\ \hline
    %%% Deit-B-dist
%    \multirow{5}{*}{DeiT-B}         & 1 & 36.0\\
%                                    & 2 & 24.2\\
%                                    & 4 & 15.2\\
%                                    & 8 & 10.2\\
    %                                & 16 & 7.4\\ \hline
%    \end{tabular}
%    \caption{Measurements of the maximum \% latency reduction obtainable by removing a single token. Larger values indicate a stronger GPU tail effect. }
%    \label{tab:max_staircase_latency_reduce}
%\end{table}
\begin{table}
    \setlength{\belowcaptionskip}{-10pt}
    \centering
    \vspace{-1em}
    \begin{tabular}{ccccc}
    \toprule
        & \multicolumn{4}{c}{Batch Size}\\
        Model & 1 & 2 & 4 & 8\\
        \toprule
        %%% Deit-B-dist
        DeiT-S & 16.1 & 19.7 & 14.6 & 10.5\\
        %%% Deit-B-dist
        DeiT-B & 36.0 & 24.2 & 15.2 & 10.2\\
        \bottomrule
    \end{tabular}
    \caption{Measurements of the maximum \% latency reduction obtainable by removing a single token on a NVIDIA Jetson TX2 for two models. Larger values indicate a stronger GPU tail effect.
    %\YHL{What is the hardware? What is the dataset?} \NJE{Added hardware - this data does not depend on dataset, so i omit that}
    }
    \label{tab:max_staircase_latency_reduce}
\end{table}

==> tables/table_similar_latency.tex <==
\begin{table}[!ht]
    \centering
    \setlength{\tabcolsep}{4pt}
    \setlength{\belowcaptionskip}{-8pt}
    %%% Device, Model + Wrapper, Accuracy, Latency
    \begin{tabular}{llllrrr}
        \toprule
        \textbf{Device} & \textbf{Batch} & \textbf{Model \&} & ~ & $\downarrow$\textbf{Acc.} & $\downarrow$\textbf{Median}\\
        ~ & \textbf{Size} & \textbf{Method} & ~ & \textbf{Loss} & \textbf{Latency (ms)}\\

        \toprule
        %%%
        %%% Jetson TX2
        %%%
        %%% Batch Size 2
        %%% DeiT-B
         \multirow{5}{*}{TX2} & \multirow{5}{*}{2} & DeiT-B & ~ & ~ & \phantom{-(00.0\%)} 215.0\\
         & & w/ Top-K & ~ & 2.44 & \textcolor{blue}{(-33.5\%)} 143.0\\
         & & w/ ToMe  & ~ & 1.63 & \textcolor{blue}{(-33.7\%)} 142.7\\
         & & w/ DyViT & ~ & \ding{61} 0.57 & \textcolor{blue}{(-33.2\%)} 143.7\\
         & & w/ Ours  & ~ & 1.16 & \textcolor{blue}{(-32.1\%)} 146.0\\
         \midrule
        %%% DeiT-S
         \multirow{5}{*}{TX2} & \multirow{5}{*}{2} & DeiT-S & ~ & ~ & \phantom{-(00.0\%)} 68.92\\
         & & w/ Top-K & ~ & 4.30 & \textcolor{blue}{(-27.0\%)} 50.32\\
         & & w/ ToMe  & ~ & 2.47 & \textcolor{blue}{(-23.1\%)} 52.98\\
         & & w/ DyViT & ~ & \ding{61} 0.46  & \textcolor{blue}{(-26.2\%)} 50.88\\
         & & w/ Ours  & ~ & 1.24 & \textcolor{blue}{(-28.3\%)} 49.44\\
        \midrule
        %%%
        %%% AGX Orin
        %%%
        %%% Batch Size 2
        %%% DinoV2-G
        \multirow{4}{*}{Orin} & \multirow{4}{*}{2} & DinoV2-G & ~ & ~ & \phantom{-(00.0\%)} 155.5\\
         & & w/ Top-K & ~ & 45.66 & \textcolor{blue}{(-32.9\%)} 104.4\\
         & & w/ ToMe & ~ & 6.96 & \textcolor{blue}{(-32.9\%)} 104.4\\
         & & w/ Ours & ~ & 2.04 & \textcolor{blue}{(-33.1\%)} 104.1\\
        \midrule
        %%%
        %%% A100
        %%%
        %%% Batch Size 2
        %%% DinoV2-G
        \multirow{4}{*}{A100} & \multirow{4}{*}{4}  & DinoV2-G & ~ & ~ & \phantom{-(00.0\%)} 40.53\\
         & & w/ Top-K & ~ & 13.31 & \textcolor{blue}{(-16.7\%)} 33.76 \\
         & & w/ ToMe & ~ & 6.96 & \textcolor{blue}{(-16.6\%)} 33.79 \\
         & & w/ Ours & ~ & 2.04 & \textcolor{blue}{(-20.1\%)} 32.37 \\
        \bottomrule
    \end{tabular}
    \caption{
    Comparison with existing methods for similar latency across device and workload sizes.
    We tune the pruning hyperparameters of the compared methods so they achieve similar latency to our method.
    %Top-K and ToMe remove $r$ tokens each layer. 
    %$R$ refers to the number of tokens our method decides to prune, and $K$ is DynamicViT's keep ratio \cite{rao_dynamicvit_2021}.
    \ding{61}DynamicViT (DyViT) requires training. Other evaluated methods are training-free.
    \PJ{Please give a reason why you chose different models for each.}
    }
    \label{tab:similar_latency}
\end{table}
